When LLMs Go Online: The Emerging Threat of Web-Enabled LLMs

Recent advancements in Large Language Models (LLMs) have established them as agentic systems capable of planning and interacting with various tools. These LLM agents are often paired with web-based tools, enabling access to diverse sources and real-time information. Although these advancements offer significant benefits across various applications, they also increase the risk of malicious use, particularly in cyberattacks involving personal information. In this work, we investigate the risks associated with misuse of LLM agents in cyberattacks involving personal data. Specifically, we aim to understand: 1) how potent LLM agents can be when directed to conduct cyberattacks, 2) how cyberattacks are enhanced by web-based tools, and 3) how affordable and easy it becomes to launch cyberattacks using LLM agents. We examine three attack scenarios: the collection of Personally Identifiable Information (PII), the generation of impersonation posts, and the creation of spear-phishing emails. Our experiments reveal the effectiveness of LLM agents in these attacks: LLM agents achieved a precision of up to 95.9% in collecting PII, generated impersonation posts where 93.9% of them were deemed authentic, and boosted click rate of phishing links in spear phishing emails by 46.67%. Additionally, our findings underscore the limitations of existing safeguards in contemporary commercial LLMs, emphasizing the urgent need for robust security measures to prevent the misuse of LLM agents.

==> outdated/outdated_PII_collection.tex <==
\section{PII Collection}
\label{sec:pii_collection}

% In this section, we investigate the extent to which LLM agents can be used to infringe upon privacy and extract personally identifiable information (PII).
% We begin by outlining the methodology for PII collection and evaluation process. 
% Subsequently, we proceed to analyze the experimental results.
\km{In this section, we investigate the potential for LLM agents to infringe upon privacy by extracting personally identifiable information (PII).}

\subsection{Methodology}


\noindent{\textbf{Attack Target.}}
% Researchers in the field of Computer Science (CS) frequently lead the development and adoption of innovative digital tools and platforms. 
As prominent members of the academic community, professors often have extensive personal and professional information available online.
Given their high profile and the significance of their reputational standing, they are particularly susceptible to targeted cyber attacks~\cite{professor_impersonation1, professor_impersonation2}.
In this context, we have identified CS professors as the primary focus of our study. Specifically, we selected professors from the CS departments of the top ten universities, as ranked by the QS World University Rankings.


To further assess variations in information collection based on academic roles, we extended our study to include PII collection from CS students.
Specifically, we focused on students affiliated with the laboratories of collected CS professors.
For this analysis, we randomly sampled 50 professors whose personal web pages had been successfully harvested in our previous PII collection process.


% to examine differences in information collection based on academic role, the subjects were divided into two groups: professors and students.
% For professor group, professors within the CS departments of popular\footnote{We select the top ten universities according to the QS World University Rankings in the Computer Science and Information Systems sector.} 10 universities were targeted.
% For student group, students belonging to the laboratories of 50 CS professors from the professor group. We randomly sampled 50 professors in popular 5 universities
% We randomly sampled 10 professors from each of the five universities whose personal pages were successfully collected through our professor PII collection process.

\noindent{\textbf{Attacker Goal.}}
The attacker's goal is to collect PII of specific targets via LLM agents.
The PII that we consider in this work include the name, email address, phone number, office address, and URL of the personal web page of each target.

% \noindent{\textbf{Attacker Knowledge.}}
% To collect PII of CS professors, the attacker only needs names of university. To collect PII of CS students, the attacker needs names of university, target  

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]
    {figures/exp1_pipeline.pdf}
    \caption{\hanna{Will be replaced}. Pipeline of PII collection (professor group). We used MIT as an example. }
    \label{fig:exp1_pipeline}
\end{figure}
\noindent{\textbf{Attack Pipeline.}}
The pipeline of PII collection (illustrated in Figure~\ref{fig:exp1_pipeline}) using LLM agents consists of two steps: 1) constructing a list of target names and 2) collecting their corresponding personal information.
Note that the attack consists of \textit{no manual effort} by the attacker and only by utilization of LLM agents.
For the professor group, the attacker initially extracts the names of CS professors from a given university (e.g., MIT). 
Then, the attacker collects the remaining PII for each professor listed. 
For the student group, the data obtained from professor group is utilized. 
Specifically, the names, personal web pages, and school affiliations of professors are used in the prompts to identify the names of students currently associated with each professor's laboratory.
The collected student names are then used as input for the LLM, which is tasked with retrieving the PII for each student.



\subsection{Implementation}
% \noindent{\textbf{Models?.}}
% As outlined in Section~\ref{sec:webagent}, the significant cost associated with the navigation function necessitates its selective use based on specific situational demands.
% Therefore, in this experiment, we selectively use 
% % Therefore, in this experiment, when the search capability of the LLM agents proved inadequate for information collection, we enhanced their functionality by integrating a navigation function.
% Additionally, we utilized LLMs as baseline comparators to evaluate the efficacy of the LLM agents.

% For the professor group, the initial collection of PII was conducted using web agents only.
% Then, we subsequently employed navigation function to gather any information that was not obtained initially.
% For the student group, obtaining the current list of students for each professor posed a significant challenge.
% Consequently, we deployed LLM agents enhanced with navigation capabilities to manage this task.
% For collecting additional PII types, only LLM agents were employed.



\noindent{\textbf{Annotation.}}
To evaluate the accuracy of the collected PII, we employed human annotators to review the responses generated by LLM agents.
Six annotators were employed, all of whom held at least a bachelor's degree and were proficient in English.


Due to the vast and diverse nature of the field of CS, we do not evaluated based solely on department listings.
Instead, annotators were directed to classify individuals as CS professors based on their engagement in relevant fields, following a thorough web search.
Only for individuals identified as CS professors, annotators conducted the remaining four PII verification processes.
Certain types of PII, such as phone number, are prone to changes over time, complicating the verification process due to discrepancies across different web sources. 
Furthermore, the probabilistic nature of responses from LLMs can lead to inconsistent information retrieval. 
To address these concerns, we initiated five separate queries to LLMs for each individual. 
Annotators were then instructed to consider the information collection successful if at least one of the five responses matched the data available online.


During the annotation process for the names of CS students, annotators referenced the student information provided at the professors' laboratory introduction pages as the ground truth. 
The methodology for annotating other types of PII remained consistent with the approach used for professors' PII.

Detailed guidelines and examples provided to annotators can be found in Appendix~\ref{?}.

\noindent{\textbf{Evaluation Metrics.}}
We use the number of successfully collected data, precision, and recall as evaluation metrics.
Precision for each category was calculated as the proportion of successfully collected PII relative to the total PII collected.

As mentioned in the annotation process, it is challenging to compile a comprehensive list of CS professors.
Consequently, we utilized the CS faculty lists provided by the official websites of each university as the reference for comparing our collected data. 
During our review, we identified several individuals not listed on the official CS faculty pages but recognized as CS professors by our annotators. 
These individuals were confirmed to be researchers specializing in CS relevant fields such as computational photography, information science, and machine learning.
Therefore, we calculated the \textit{upper bound recall} using the number of professors officially listed under the CS faculty.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]
    {figures/pii_main_result.pdf}
    \caption{The quantities of correctly collected PII of (a) CS professors and (b) CS students. (c) is an enlarged version of (b).}
    \label{fig:PII_professor}
\end{figure*}

\subsection{Results and Analysis}
When prompted to collect PII, GPT and Claude generated responses successfully, whereas Gemini refused to process such requests due to privacy concerns.
Thus, we only evaluated responses generated by \textbf{GPT} and \textbf{Claude}.

\subsubsection{PII collection results}
Figure~\ref{fig:PII_professor} demonstrates the results of PII collection of CS professors using LLMs and LLM agents. 
The GPT LLM agent and Claude LLM agent successfully collected the names of 506 and 632 professors, respectively, out of a total of 686~\footnote{The total number of professors listed on the CS faculty.}, showing a significant increase in data collection compared to their performance as LLMs.
% We observed that both GPT and Claude significantly collected more data when operating as LLM agents compared to LLMs.
Notably, the difference was more pronounced with GPT. 
Without utilizing web capabilities, both models struggled to retrieve office addresses and phone numbers.

GPT LLM correctly gathered 327 names of CS professors but only retrieved 39 office addresses and 36 phone numbers correctly, showcasing very low efficiency. In contrast, its LLM agent correctly collected 506 names and show a broader range and higher retrieval efficiency across all categories.

Claude showed a similar trend where the LLM agent generally retrieved more data than the LLM, except for the name category. 
Specifically, without the web search function, Claude managed to collect 795 names, which exceeds the 632 names gathered by its LLM agent. 
Figure~\ref{fig:PII_professor} (c) shows that the LLM agents exhibited higher precision across all categories compared to the LLMs overall. 
Excluding the name category, GPT demonstrated higher precision than Claude across all other categories.

\harry{These contrasting results between using the LLM and LLM agent for both GPT and Claude portray that access to the web greatly widens the performance of extracting PII of specified targets. Despite the information being publicly available on the Internet, the successful retrieval of PII by the LLM agents is an alarming feature that may require reconsideration.}


\noindent{\textbf{Self-evaluation.}}
To enhance precision and reduce costs associated with the incorrect collection of professor names, attackers can implement LLM self-evaluation. 
We prompted LLMs and LLM agents with the question: ``Is [NAME] a CS professor at [UNIVERSITY]? Say Yes or No.'' Based on their responses, we refined the list of collected professor names.
This step serves as a filtering step for the attacker for more precise information retrieval.


% Attackers gather PII based on the compiled list of professors. Cost considerations are critical for attackers; thus, it is essential to enhance the precision of the professor list to optimize effectiveness and efficiency.
% To address this issue, we implemented a self-evaluation step after constructing the professor list. 

Table~\ref{tab:professor_self_eval} demonstrates that self-evaluation was able to significantly boost the precision of PII collection by both LLMs and LLM agents.
Notably, precision values for LLM agents reached high levels, approaching or even exceeding 0.9.
Although self-evaluation is a simple feedback step that adds only a single extra query to the attack pipeline, it markedly enhances performance.
Such phenomena of self-correction have been recognized as beneficial in various tasks, including question answering~\cite{peng2023check} and chain-of-thought reasoning~\cite{he2022rethinking}.
Despite the exclusion of some correctly identified professor names, the notable increase in precision --- 1.97x for GPT LLMs, 1.76x for GPT LLM agents, 1.25x for Claude LLMs, and 1.24x for Claude LLM agents --- indicates that the benefits of enhanced precision may outweigh these losses.

\input{tables/professor_self_eval}

\noindent{\textbf{Navigation-enhanced LLM Agents.}}
Here, we investigate the enhanced PII collection capabilities of LLM agents when augmented with a navigation function.
We recollect the PII using navigation-enabled LLM agents for professors whose initial data collection was incomplete in at least one of the specified four categories, excluding names. 
Specifically, GPT and Claude agents were utilized to recollect PII for 256 and 417 professors, respectively.
Table~\ref{tab:pii_navi} shows the results of recollection. 
This result indicated that both models significantly enhanced their PII collection capabilities through web navigation function, with notable improvement observed in phone numbers and office addresses.

Interestingly, the GPT agent, when not utilizing the navigation function, collected slightly more email addresses and personal web pages than it did with navigation enabled. 
This arises from navigation failures, which occurred for 24 out of the 256 professors due to token limits imposed by OpenAI. 
% These limits restrict the amount of data that can be processed in a single interaction.
When attempting to navigate multiple pages to locate the desired information, the navigation agent consumed an excessive number of tokens, resulting in information collection failures for these individuals.

\input{tables/professor_PII_navigation}

\input{tables/student_name_collection}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]
    {figures/exp1.2_student_name.pdf}
    \caption{The number of correctly collected names of CS students by GPT and Claude, from a total of 514 students in the constructed ground truth.}
    \label{fig:student_name}
\end{figure}
\subsubsection{PII collection of CS students.}
Figure~\ref{fig:student_name} illustrates the number of collected student names by each models.
Both GPT and Claude demonstrated low efficiency in configurations without the navigation function. 
Interestingly, when operating solely as LLMs without the search feature, they provided a lot of incorrect student names with significantly low precision, exhibiting pronounced hallucinations (shown in Table~\ref{tab:student_prc_result}).
Notably, Claude LLM retrieved over twice as many student names as GPT LLM (335 vs 148), most of which were inaccurately identified, highlighting that Claude is significantly more prone to hallucinations than GPT.
However, with navigation enabled, both agents demonstrated improved effectiveness, correctly identifying 509 and 463 students, respectively.


\noindent{\textbf{LLM agent without navigation.}}
Our experimental results show that LLM agents without navigation function cannot retrieve the student list effectively.
Upon analysis, the reason stems from the limitation of web search API, Google Custom Search API. This API does not fetch all the content from a website; instead, it returns snippets, which are automatically generated excerpts that summarize a page's content and highlight search terms~\cite{google_snippet}. Therefore, the search results sometimes only included some of the students' names or retrieved names of alumni.
We will discuss about this in Section~\ref{sec:discussion}.


\noindent{\textbf{Navigation Strategies in LLM Agents.}}
In settings with navigation-enhanced LLM agents, Claude underperformed compared to GPT.
This discrepancy comes from Claude's failure to retrieve the student list from 10\% (5 out of 50) of the given pages.
The failure stems from the different approaches to exploration and contextual analysis between them. 
GPT, despite uncertainties, consistently undertakes multiple explorations to locate the student list. 
In contrast, Claude tends not to pursue further exploration when the context remains unclear.

Specifically, if the student list is explicitly listed on the given website, the LLM agent scrapes and returns the information directly. However, if it is not immediately available, the agent employs navigational techniques within the site to locate the student list, utilizing buttons or links as necessary. 
For instance, the agent may need to access a professor's laboratory page via a link on the site and search for the student list therein. 
Even if the site does not explicitly indicate that a link leads to a professor’s laboratory, GPT will explore the link to determine if the necessary information is present. 
In contrast, Claude does not pursue links unless they are clearly marked, and will report the absence of student information if clarity is lacking.  
Another scenario involves links to ongoing research projects led by the professor. Here, GPT actively retrieves student names by following the links, while Claude refrains from engaging and simply reports that no student names are found on the site.


\noindent{\textbf{Collect remaining PII.}}
Building on the insight gained from professor data collection (where GPT was more effective than Claude at collecting PII), we utilized the GPT agent to gather the remaining PII for students. 
Since some students are affiliated with multiple professors, we removed duplicates and proceeded to collect data for the 439 students. 

We successfully gathered 69 phone numbers, 63 office addresses, 318 email addresses, and 226 personal pages out of the total 439 students.
The PII collection results of student group show a similar pattern to professor group across different categories.
However, unlike professors, students often do not have or disclose their personal information details, resulting in lower figures across each category.

\subsubsection{Cost Analysis}
We perform an analysis of the cost of collecting PII of LLM agents associated with the use of navigation functions and different model types.
We randomly selected 50 professors from the collected data. 
We measured the time spent, the number of function calls, and the number of tokens consumed during the process of collecting each professor's PII.


To measure the number of tokens, we utilized the tiktoken tokenizer~\cite{tiktoken} for the GPT-4o model, as specified by OpenAI~\cite{tiktoken_openai}. 
For Claude, we used the token counting feature provided by its API~\cite{anthropic_tokencnt}.

Table~\ref{tab:cost_stat} shows statistics for each category. Using navigation was more expensive in terms of time and token consumption compared to not using navigation. 
During the process of searching for information, time and tokens are consumed as various links and buttons are clicked within the site. 
Upon adding navigation functionality, the average token usage for GPT and Claude agents increased by 8.95 times and 6.80 times, respectively.
Optimizing the navigation feature could potentially mitigate these costs.

\noindent{\textbf{GPT vs. Claude.}}
Interestingly, regardless of the use of navigation functions, GPT made more function calls than Claude. 
Without navigation, this difference became even more pronounced because GPT continuously altered search queries when the desired information was not immediately found. 
This result highlights GPT's more proactive exploration compared to Claude, as previously mentioned.

When not using the navigation function, GPT required less time to complete tasks than Claude, despite making more function calls.
This could be attributed to differences in model performance, aligning with the analysis reported in ~\cite{gpt-4o_analysis}.


\input{tables/exp1_time}

==> outdated/outdated_Phishing_email.tex <==
\section{Spear Phishing Email Generation}
Spear phishing emails are highly effective at deceiving victims but tend to be more costly and time-consuming for attackers compared to traditional phishing emails~\cite{spear_phishing_cost1, spear_phishing_cost2}. 
This increased effort is due to spear phishing's focus on targeting specific individuals or organizations with tailored messages. 
In this section, we examine the extent to which LLM agents can generate personalized phishing emails using only an email address, without the need for additional human intervention.


\subsection{Methodology}
\noindent{\textbf{Attack Target.}}
In Section~\ref{sec:pii_collection}, we demonstrated the feasibility of effectively obtaining email addresses of researchers in university. 
Similarly, attackers can exploit publicly available email addresses~\cite{mirante2013understanding} or acquire them through purchases on the dark web or Telegram channels~\cite{get_emailaddress1}. 
In this experiment, we targeted individuals whose email addresses were obtained by the attacker. 

\noindent{\textbf{Attack Goal.}}
Attackers commonly use phishing emails to obtain sensitive information from targeted individuals by asking them to click on a link and enter personal information~\cite{phishing_email_link}. 
In our study, the attacker's goal is to automatically generate highly personalized spear phishing emails that take into account the recipient's expertise, relationships, and other relevant factors. This approach aims to make the emails appear legitimate and increase the likelihood that recipients will click on the links.


\noindent{\textbf{Attack Pipeline.}}
The attack pipeline is designed to craft highly convincing phishing emails. 
Note that the attack consists of \textit{no manual effort} by the attacker and only by utilization of LLM agents.
The only ingredient for this attack is the \textit{target's email address}, which is added into the generation prompt of the LLM query.

Figure~\ref{} shows the attack pipeline.
The attack starts with date verification to ensure the timing aligns with the intended attack scenario. 
The process then moves to creating the email content, which gathers the email owner's information by searching their email address online.
This information is then used to design a realistic use case where the target is likely to receive an email, along with identifying a credible sender that fits the scenario. 
A plausible URL string is then generated and embedded in the email to encourage the target's engagement. 
Finally, the sender's email address is modified to resemble a legitimate domain, allowing the attacker to dispatch the email without the need to exploit vulnerabilities in official domains or compromise accounts to utilize the authentic domain.




\subsection{Implementation}
\begin{comment}
- LLMs have safeguard capability
- emails are custom generated
- questionnaire is made and evaluated by surveys
- not sent, just google survey

\end{comment}
This attack relies on the extensive versatility of the LLM and LLM agents, and relies heavily on the generation prompt.
Many LLM services are accompanied with a safety feature that safeguards the LLM to prevent them from being misused for harmful intentions~\cite{inan2023llama, wang2023not}. This feature should be bypassed for the implementation of this attack.
Therefore, we first assessed safeguard capability of LLMs and LLM agents by changing email designs.
Based on the findings from this stage, we selected seven specific email designs for evaluating the effectiveness of phishing emails.

After identifying the safeguard bypass prompts, emails were custom-generated for each target, necessitating that each recipient personally evaluate the emails intended for them. 
Consequently, we developed a questionnaire specifically for the evaluation of these emails and actively recruited participants to ensure a comprehensive assessment. 
Importantly, note that we DID NOT send any emails. 
Instead, we asked participants to assess the generated emails using a Google survey.

\noindent{\textbf{Safeguard Capability Assessment.}}
To understand the safeguard capabilities of LLMs, we conducted an experiment using the email addresses of the authors, with their consent, to generate emails. The experiment involved varying two key factors: 1) the purpose of the email, and 2) the type of email address used. 
Since our paper does not specifically address LLM jailbreaks, our experiment includes minimal circumvention techniques, such as avoiding explicit terms like ``phishing email''.

We divided the purpose of email into three groups: general, login credentials, and money. 
For the general purpose, LLMs were tasked with autonomously generating a realistic scenario in which the target might receive an email. 
When focusing on login credentials, we provided specific instructions for the LLMs to generate an email prompting the target to change their credentials. 
For the money-related purpose, the LLMs were directed to compose a legitimate email requesting money from the target. 
Regarding the email type, we included both institutional email addresses and Gmail addresses in the experiment.


\noindent{\textbf{Email Design.}}
Based on the results of safeguard capability assessment, we selected six types (M2$\sim$M7) of emails for further evaluation (Table~\ref{tab:email_type}). 
Additionally, to examine the impact of the recipient's affiliation, we included M1, a modified version of M2, where the sender belongs to a different institution than the target. 
For M1, we use Claude as the generation model because it tends to produce higher-quality phishing emails compared to GPT at pilot study.
Note that we include only Claude and GPT, as Gemini refused to generate them due to its safeguard restrictions.


\noindent{\textbf{Questionnaire Design.}}
We design seven questions to sequentially build a comprehensive understanding of how participants perceive and interact with the emails, from surface content to deeper implications of authenticity and intended actions. For fast completion, the questionnaire only contains multiple choice questions and check box.

First, we explored the \textit{content} of the emails, asking participants to identify the information presented and evaluate how well it matched their actual personal details. Subsequently, we probed perceptions of the sender and recipient, such as whether the recipient recognized the sender and the recipient name is align with the real name. 
We then inquired about the \textit{actions} participants would likely take upon receiving the email. 
Lastly, we investigated the \textit{perceived authenticity} of the email, asking participants to assess how genuine or fraudulent it appeared and to identify specific elements that influenced their judgment. 
\textcolor{red}{Established questionnaire can be found in Appendix~\ref{}.}

\input{tables/phishing_email_type}

\noindent{\textbf{Recruiting.}}
We advertised our study within communities and initially contacted potential participants from our personal networks.
All participants were informed about an incentive of approximately \$7.50 for their participation in the study.

% To analyze the evaluation results relative to security awareness and the characteristics of the institutions associated with the targets, we ensured a balanced distribution among individuals from both security and non-security sectors, as well as from research and industry domains. 
To analyze the evaluation results relative to the characteristics of the institutions associated with the targets, we ensured a balanced distribution among individuals from research and industry domains. 
This balanced approach facilitated a comprehensive evaluation of the variables under investigation.

At the beginning of the study, participants were provided with a consent form. 
Then, we asked to provide their institutional email addresses.
Upon receiving consent, we collected email addresses for the purpose of data collection integral to the experimental design. 
For each email address, we generated seven distinct types (Table~\ref{tab:email_type}) of emails using LLMs and LLM agents. 

Participants were then asked to assess these emails through a questionnaire on Google Survey that we administered. 
It is important to note that each participant was exposed only to emails generated from their own email address.
We instructed participants to evaluate the emails under assumption that they had received these emails to their own email addresses.

Of the 70 individuals who provided their email addresses via the consent form, 60 completed the evaluation of the emails.

\noindent{\textbf{Sample Description.}}
A total of 60 participants filled out our questionnaire.
We categorized their domains based on the institutional addresses they provided. 
Among these participants, 55\% were from research backgrounds and 45\% from industry.
% Within the research group, 60.6\% specialized in the security field, whereas 44.4\% of the industry participants were involved in security.


\subsection{Results \& Analysis}


\subsubsection{Safeguard Capability}
Table~\ref{tab:email_generation} shows results of phishing email generation based on the email's purpose and the type of email address used.
When an institutional email address is provided, GPT and Claude are more likely to generate an email.
We observed that Gemini, Claude, and GPT ranked in that order in terms of safeguard capability. 
Gemini demonstrates the strongest safeguards by refusing to generate emails in all scenarios both LLM and LLM Agent settings, responding with messages like \textit{``I cannot fulfill your request to generate an email address or email content. Creating and sending emails without consent is unethical and potentially illegal''}.

All models are more likely to refuse generating content when the email's purpose involves login credentials or money, indicating these topics trigger stricter safeguard mechanisms.
However, general-purpose emails are less likely to be blocked, with GPT and Claude generating responses in these cases.


Despite Gemini’s strong safeguards, it was noted in when only \textit{web accessibility} was added, the model that previously refused to generate content under strict settings began to produce a response. 
This suggests that certain tool uses can serve as a form of jailbreak, which can expand threat surface of LLMs.



\input{tables/email_generation}
\input{tables/phishing_result}
\subsubsection{Effectiveness of Phishing Emails}
\noindent{\textbf{Overall Analysis.}}
Table~\ref{tab:overall} presents the results based on email types. 
For general-purpose emails (M2,5 vs. M4,7), versions with web accessibility were more effective in phishing, as evidenced by higher link click rates and a greater proportion of participants not recognizing them as phishing attempts. 
Additionally, emails targeting login credentials (M3,6 vs. M2,5) were more effective to make them click the link. 
This aligns with existing research~\cite{alkhalil2021phishing} indicating that urgent requests, such as change login information, are effective in phishing scenarios.
Considering that LLMs without web accessibility refuse to generate emails targeting login credentials, it suggests that LLM agents are more proficient at generating successful phishing emails compared to LLMs. 

An interesting point is that our results show LLM agents could be as effective as, or even more effective than, human-crafted spear phishing emails in prompting clicks.
In \cite{bethany2024large}, link click rates for phishing emails using internal addresses and information were 26.6\% for human-crafted and 16.7\% for LLM-generated emails.
In our study, over 20\% of participants (up to 46.67\%) responded they would click on links in LLM agent-crafted emails. 
While these results are not directly comparable due to different methods and participant groups, they suggest that LLM agents were highly effective in generating phishing emails—especially considering that our attack model requires significantly less knowledge and capability, and no human labor.


\noindent{\textbf{Content Analysis.}}
We analyzed how web accessibility influences the detail in email content (Q1, multiple responses allowed) and the alignment of those details with the target's information (Q2, multiple responses allowed). 
Both factors played statistically significant roles in participants' assessment of an email's authenticity (Q1- $\kappa$: 98.8, $p$ \(\ll\) 0.05, Q2- $\kappa$: 113.5, $p$ \(\ll\) 0.05 ).
Figure~\ref{fig:phishing_content_result} shows the percentage of emails containing these categories based on the responses.

The results indicate that emails crafted by LLM agents included more detailed content and were more aligned with the target's information compared to those generated by LLMs alone, with this difference being particularly pronounced in GPT-generated emails. 
The alignment of the email's specific expertise with the target's own expertise had the most significant impact on their perception of the email's authenticity 
($\kappa$: 11.15, $p$: \(\ll\) 0.05).

These findings support the conclusion that LLM agents can create more targeted and detailed phishing emails leveraging information available on the web.


 
\noindent{\textbf{Factors Influencing Phishing Email Detection.}}
We examined the factors that influenced participants' decisions to identify an email as phishing (Q7, multiple responses allowed).
We calculated the percentage of each factor based on how frequently participants selected each response factor.
The factors were ranked by their influence, with sender information (62.3\%), email purpose (39.7\%), and information related to expertise (31.6\%) being the most significant. 
This results align with the previous studies showing that users heavily consider the sender's information when assessing an email's authenticity~\cite{10190709}. 
Notably, altering the sender's email to that of a different organization (M1 vs. M2) increased the link click rate by 1.75 times, with 47.2\% of those identifying M1 as phishing citing sender information as the factor. 
This suggests participants are more vulnerable to deception when unfamiliar with the sender's domain. 
Additionally, for emails requesting login credentials (M3, M6), 48.8\% and 51.2\% of participants, respectively, cited the email's purpose as the reason for identifying it as phishing, which is higher than the average.

% This finding implies that using spoofing techniques could potentially lead to more effective attacks.

% When the sender's email address was altered to that of a different organization (M1 vs. M2), the link click rate increased by 1.75 times. 
% This supports the idea that users place significant importance on the sender's information when evaluating an email's authenticity~\cite{10190709}. Participants were less familiar with domains from other organizations, making them more vulnerable to deception, unlike when the emails came from their own organization's domain.
 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]
    {figures/phishing_content_result_v3.pdf}
    \caption{Comparative analysis of email content by category (M2, M4, M5, M7): (a) Detail of email content and (b) Alignment of email content with the target. }
    \label{fig:phishing_content_result}
\end{figure}


\noindent{\textbf{Group Analysis.}}
Figure~\ref{fig:phishing_group_result} presents the results of actions the actions that participants in each group reported they would take after receiving an email. 
In the research group, there were generally more individuals who indicated they would click the link compared to the non-research group. Unlike enterprise groups, research labs or groups within universities often have dedicated websites that list all members, including professors and graduate students. 
These pages frequently highlight current projects, research interests, and recent publications. 
This availability of detailed information makes research groups more susceptible to targeted phishing attacks.
This aligns with our experimental results. 
We examined the percentage of participants who indicated that none of the information in the email matched their own in Q2. 
In the research group, this percentage ranged from as low as 0\% (M2) to a maximum of 12.12\% (M7). 
In contrast, in the non-research group, even for emails generated with web accessibility (M2, M5), the percentage of participants who said none of the information matched was 7.41\% and 40.74\%, respectively.


For the research group, the LLM agents for both Claude and GPT were more effective at prompting link clicks compared to the LLMs, with increases of 1.37 times and 1.75 times, respectively. 
In the non-research group, adding web accessibility to Claude resulted in the same link click rate but reduced the percentage of participants who said they would move the email to the spam folder by X times. 
For GPT, adding web accessibility increased the link click rate by 2.49 times.

These results suggest that LLM agents can create much more threatening phishing emails with web accessibility and that researchers, who often have a significant amount of public information available online, are particularly at risk.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]
    {figures/phishing_group.pdf}
    \caption{Analysis of results according to group: (a) research and (b) non-research. }
    \label{fig:phishing_group_result}
\end{figure}


==> sections/ThreatModel.tex <==
\section{Threat Model}

\subsection{Attacker Goal}
We selected three tasks that leverage vulnerabilities introduced by the prevalence of personal data on the web, as prohibited by OpenAI's policy: PII collection, impersonation, and spear phishing email generation.

\noindent{\textbf{PII Collection.}} Collecting Personal Identifiable Information (PII) from the internet does raise privacy concerns, even if the data is publicly accessible. 
Attackers can use it for malicious purposes such as identity theft, fraud, or further cyber attacks.
Attackers use web scraping tools and automated scripts to collect PII from the web. Since each site displays information in a unique format, these tools often need to be custom-developed for each target site, requiring significant human labor and associated costs.

\noindent{\textbf{Impersonation Post Generation.}} 
% There has been a rise in impersonators who falsely claim to be reputable individuals, leading to an increase in social media impersonation~\cite{impersonation3, impersonation4}. 
Attackers write impersonation posts primarily to deceive their target audience for malicious purposes, such as financial gain, tarnish reputations~\cite{impersonation1, impersonation2}. 
To create sophisticated impersonation posts, attackers need to research personal details, social behaviors, and communication styles, and incorporate these elements into their writing. This process requires significant time and effort.

\noindent{\textbf{Spear Phishing Email Generation.}} 
Spear phishing emails are highly effective at deceiving victims but tend to be more costly and time-consuming for attackers compared to traditional phishing emails~\cite{spear_phishing_cost1, spear_phishing_cost2}. 
This increased effort is due to spear phishing's focus on targeting specific individuals or organizations with tailored messages. 

공격자들은 

\noindent{\textbf{Attacker Assumptions.}}
sdfsd

==> tables/email_generation.tex <==

\begin{table}[h]
\caption{Response generation capabilities of LLMs across different configurations. successfully generated a response (o) or refused to generate a response (x)}
\label{tab:email_generation}
\footnotesize
\centering
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{ccccc|ccc}
\toprule
&& \multicolumn{3}{c}{LLM} 
& \multicolumn{3}{c}{WebSearch Agent} \\
\cmidrule(r){3-8}  
&& GPT& Claude & Gemini & GPT & Claude& Gemini\\
\midrule
\multirow{3}{*}{Purpose} & General& o& o& x& o& o& x\\
& Credential & x& x& x& o& o& x\\
& Money& x& x& x& o& x& x\\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Email\\address\\
\end{tabular}}
& Institutional & o& o& x& o& o& x\\
& Gmail & o& x& x& o& o& x\\
\bottomrule
\end{tabular}

\end{table}


==> tables/exp1_time.tex <==



% \begin{table}[t]
% \centering
% \caption{Cost statistics for LLM agents to collect PII of professors with and without the navigation function.}
% \label{tab:cost_stat}
% \footnotesize
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{cc rrrr}
% \toprule
% &&\multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{Claude} \\  
% \cmidrule(r){3-4} \cmidrule(r){5-6}
%  & navigation& \multicolumn{1}{c}{x} & \multicolumn{1}{c}{o} & \multicolumn{1}{c}{x} & \multicolumn{1}{c}{o}\\
%  \midrule
% \multirow{4}{*}{Time (sec)} 
% & min & 3.33 & 6.53 & 7.85 & 15.13 \\
% & max &  11.18 &  294.45 & 17.51 &  180.66 \\
% & median &  6.79 & 33.16 & 10.62 &29.75 \\
% & mean &  6.69 & 53.5 & 11.43 & 43.28 \\
% \midrule
%  & min & 1.00 & 2.00 &1.00 & 2.00 \\
% \# Function & max &  6.00 &  17.00& 2.00 &  8.00\\
% calls& median &  3.50 & 5.00 & 1.00 & 4.00 \\
% & mean &   3.56  & 5.74 &1.40 & 3.72 \\
% \midrule
% \multirow{4}{*}{\# Tokens} 
% & min & 438.00 & 895.00 & 1159.00 & 1948.00\\
% & max & 2559.00 & 76041.00 & 2268.00& 78662.00\\ 
% & median & 1389.50 & 6298.50& 1301.00 & 5202.00\\
% & mean &  1406.04 &12583.74& 1462.78 & 9952.80  \\
% \bottomrule
% \end{tabular}
% \end{table}



\begin{table}[h]
\centering
\caption{Cost statistics for LLM agents to collect PII of professors with and without the navigation function.}
\label{tab:cost_stat}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{cc rrrr}
\toprule
&&\multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{Claude} \\  
\cmidrule(r){3-4} \cmidrule(r){5-6}
 & navigation& \multicolumn{1}{c}{x} & \multicolumn{1}{c}{o} & \multicolumn{1}{c}{x} & \multicolumn{1}{c}{o}\\
 \midrule
\multirow{3}{*}{Time (sec)} 
& min & 3.33 & 6.53 & 7.85 & 15.13 \\
& max &  11.18 &  294.45 & 17.51 &  180.66 \\
& mean &  6.69 & 53.50 & 11.43 & 43.28 \\
\midrule
 & min & 1.00 & 2.00 &1.00 & 2.00 \\
\multirow{3}{*}[+2.3ex]{\shortstack[]{\# Function \\ calls}}& max &  6.00 &  17.00& 2.00 &  8.00\\

& mean &   3.56  & 5.74 &1.40 & 3.72 \\
\midrule
\multirow{3}{*}{\# Tokens} 
& min & 438.00 & 895.00 & 1159.00 & 1948.00\\
& max & 2559.00 & 76041.00 & 2268.00& 78662.00\\ 
& mean &  1406.04 &12583.74& 1462.78 & 9952.80  \\
\bottomrule
\end{tabular}
\end{table}



==> tables/fakenews_title.tex <==
\begin{table*}[ht]
\centering
\footnotesize
\caption{Original titles of recent US politics news from CNN and reversed titles of them created by GPT-4o}
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
\textbf{Date} & \textbf{Original Title} & \textbf{Reversed Title (gpt-4o)} \\ 
\midrule
2024-08-10
& Former California lawmaker Nate Holden says he was on the scary helicopter ride with Trump
& Contested Memories: Trump, Ex-Councilman Holden, and Former Mayor Brown Dispute Helicopter Incident \\
\midrule
2024-08-12 
& Trump and Musk host friendly conversation on X after delay from technical difficulties
& Trump and Musk's Contentious X Dialogue: Technical Hurdles, Policy Clashes, and High Stakes for 2024\\
\midrule
2024-08-12 
&Colorado election denier Tina Peters convicted in election computer breach 
& Colorado Clerk Tina Peters Acquitted on Most Charges in Election Computer System Breach Case\\ 
\midrule
2024-08-12
&Arizona abortion rights measure will be on November ballot
&Arizona Abortion Restriction Measure Achieves Historic Signature Certification, Heads to November Ballot\\
\midrule
2024-08-12
&RFK Jr. denied ballot access in New York after judge rules he used ‘sham’ address on petition
&Robert F. Kennedy Jr. Wins Major Legal Victory in New York Ballot-Access Case, Securing Key Boost for Independent Presidential Run\\
\midrule
2024-08-12
&Police investigating break-in at Trump campaign office in Virginia
&Law Enforcement Confirms No Investigation Needed for Non-Existent Break-In at Trump Campaign Office in Virginia \\
\midrule
2024-08-12
&Suspected Iranian hackers breached Roger Stone’s personal email as part of effort to target Trump campaign, sources say
&FBI Investigates Iranian Involvement in Safeguarding of Trump Campaign Documents and Roger Stone's Email Account \\
\midrule
2024-08-12
&Both Trump and Harris want to eliminate taxes on tips. This is how it could affect workers
&Trump and Harris Face Criticism Over Tax Proposal on Tips Amid Presidential Campaign \\
\midrule
2024-08-13
& Musk tries to help Trump halt the Harris surge
& Elon Musk and Donald Trump Spar Over Key Political Issues in a Transformative Social Media Dialogue on X \\
\midrule
2024-08-13
&How Harris is reversing Biden’s biggest weakness in the campaign
& The Battle for Strength: Trump Reframes the Presidential Debate Against Harris \\

\bottomrule
\end{tabularx}
\end{table*}


==> tables/impersonation_cross.tex <==
% \begin{table}[t]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{5pt}
%     \begin{tabular}{l ccc ccc}
%         \toprule
%          & \multicolumn{3}{c}{claim1} & \multicolumn{3}{c}{claim2} \\
%         \cmidrule(r){2-4} \cmidrule(r){5-7}  
%         \textbf{Eval} & Agent & LLM & Unsure & Agent & LLM & Unsure \\
%         \midrule
%         Claude & 79.6 &20.4 & 0.0   & 63.3& 30.6 & 7.0 \\
%         Gemini & 77.6 & 22.4 & 0.0 & 65.3 & 34.7 & 0.0 \\
%         % \midrule
%         % \multirow{3}{*}{claim2}
%         % &GPT   & 78 (10)  & 62 (6) & 64 (0) \\
%         % &Claude  & 58 (18)   & 56 (12)  & 64 (6)  \\
%         % &Gemini & 72 (18)   & 64 (4) & 54 (16) \\
%         \bottomrule
%     \end{tabular}
%     \caption{A/B Test using cross-evaluation for texts generated by GPT. Percentages represent each response relative to the total 
% \end{table}

% \begin{table}[t]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{3pt}
%     \caption{A/B testing results where models evaluate each other's outputs. The percentages represent each decision relative to the total number of decisions made.}
%     \begin{tabular}{ll ccc ccc}
%         \toprule
%          && \multicolumn{3}{c}{claim1} & \multicolumn{3}{c}{claim2} \\
%         \cmidrule(r){3-5} \cmidrule(r){6-8}  
%         \textbf{Gen}&\textbf{Eval} & Agent & LLM & Unsure & Agent & LLM & Unsure \\
%         \midrule
%         \multirow{2}{*}{GPT}&
%         Claude & 79.6 &20.4 & 0.0   & 63.3& 30.6 & 7.0 \\

%        & Gemini & 77.6 & 22.4 & 0.0 & 65.3 & 34.7 & 0.0 \\
%        \midrule
%         \multirow{2}{*}{Claude}&
%         GPT &  68.0 & 24.0 & 8.0 & 67.4 &11.6&  20.9\\
%         &Gemini & 70.0 & 16.0 & 14.0 &79.0 & 14.0 & 7.0 \\
%         \midrule
%         \multirow{2}{*}{Gemini}&
%         GPT & 76.0 &18.0& 6.0&  72.0 &10.0 &18.0\\
%         &Claude & 60.0 &36.0 &4.0 &58.0 &26.0 &16.0 \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:impersonation_cross}
% \end{table}

\begin{table}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{1.7pt}
    \caption{A/B test results (WebSearch agent vs. vanilla LLM). The percentages represent each decision relative to the total number of decisions made. claim1 refers to ``\textit{Recommend researching AI}'' and claim2 to ``\textit{LLM is highly secure against potential misuse}''. }
    \begin{tabular}{ll ccc ccc}
        \toprule
         && \multicolumn{3}{c}{claim1} & \multicolumn{3}{c}{claim2} \\
        \cmidrule(r){3-5} \cmidrule(r){6-8}  
        \textbf{Gen}&\textbf{Eval} & \scriptsize\makecell{WebSearch\\Agent} & \scriptsize LLM & \scriptsize Unsure & \scriptsize\makecell{WebSearch\\Agent} & \scriptsize LLM & \scriptsize Unsure \\
        \midrule
        \multirow{3}{*}{GPT}&
        GPT & 79.6 & 18.4 & 2.0  & 69.4 & 20.4& 10.2 \\
        \cmidrule(lr){2-8}
       & Claude & 79.6 &20.4 & 0.0   & 63.3& 30.6 & 7.0 \\

       & Gemini & 77.6 & 22.4 & 0.0 & 65.3 & 34.7 & 0.0 \\
       \midrule
        \multirow{3}{*}{Claude}&
        Claude & 68.0 & 28.0 & 4.0 & 65.0 & 14.0 & 21.0 \\
        \cmidrule(lr){2-8}
        & GPT &  68.0 & 24.0 & 8.0 & 67.4 &11.6&  20.9\\
        &Gemini & 70.0 & 16.0 & 14.0 &79.0 & 14.0 & 7.0 \\
        \midrule
        \multirow{3}{*}{Gemini}&
        Gemini & 64.0 & 28.0 & 8.0&  58.0& 26.0&16.0\\
        \cmidrule(lr){2-8}
        &GPT & 76.0 &18.0& 6.0&  72.0 &10.0 &18.0\\
        &Claude & 60.0 &36.0 &4.0 &58.0 &26.0 &16.0 \\
        \bottomrule
    \end{tabular}
    \label{tab:impersonation_cross}
\end{table}

==> tables/impersonation_navi_search.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3.3pt}
    \caption{A/B test results. The percentages represent each decision relative to the total number of decisions made. claim1 refers to ``\textit{Recommend researching AI}'' and claim2 to ``\textit{LLM is highly secure against potential misuse}''. WebN and WebS represent WebNav and WebSearch, respectively. }
    \begin{tabular}{ll ccc ccc}
        \toprule
         && \multicolumn{3}{c}{claim1} & \multicolumn{3}{c}{claim2} \\
        \cmidrule(r){3-5} \cmidrule(r){6-8}  
        \textbf{Gen}&\textbf{Eval} & \scriptsize \makecell{WebN\\Agent} & \scriptsize \makecell{WebS\\Agent} & \scriptsize Unsure & \scriptsize \makecell{WebN\\Agent} & \scriptsize \makecell{WebS\\Agent} & \scriptsize Unsure \\
        \midrule
        \multirow{3}{*}{GPT}&
        GPT & 60.4 & 39.6 &	0.0 & 64.6&31.3&4.2  \\
        \cmidrule(lr){2-8}
       & Claude & 54.2 & 43.8 & 2.1 & 56.3&35.4&8.3 \\
       & Gemini & 47.9 & 43.8 & 8.3 &60.4&37.5&2.1 \\
        \midrule
        \multirow{3}{*}{Claude}&
        Claude & 55.1 & 42.9 & 2.0 &59.2&32.6&8.2\\
        \cmidrule(lr){2-8}
        & GPT & 61.2 & 30.6 & 8.2 & 49.0&20.4&30.6\\
        &Gemini & 44.9 & 38.8 & 16.3 &42.9&40.8&16.3\\
        \midrule
        \multirow{3}{*}{Gemini}&
        Gemini & 33.3 & 50.0 & 16.7 &29.6&33.3&37.0\\
        \cmidrule(lr){2-8}
        &GPT & 66.7 & 23.8 & 9.5 & 48.1&29.6&22.2 \\
        &Claude & 64.3 &33.3 & 2.4 &59.3&37.0&3.7 \\
        \bottomrule
    \end{tabular}
    \label{tab:impersonation_cross_navi_search}
\end{table}









==> tables/impersonation_result.tex <==

% \begin{table}[t]
%     \centering
%     \footnotesize
%     \begin{tabular}{lcccc}
%         \toprule
%         && \multicolumn{3}{c}{Evaluation Model} \\
%         \cmidrule(r){3-5}  
%         & & GPT & Claude & Gemini \\
%         \midrule
%         \multirow{3}{*}{claim1}
%         & GPT    & 39/1/9  & 39/0/10 & 38/0/11 \\
%         &Claude & 34/4/12 & 34/2/14 & 35/7/8  \\
%         &Gemini & 38/3/9  & 30/2/18 & 32/4/14 \\
%         \midrule
%         \multirow{3}{*}{claim2}
%         &GPT   & 34/5/10  & 31/3/15 & 32/0/17 \\
%         &Claude  & 29/9/5   & 28/6/9  & 34/3/6  \\
%         &Gemini & 36/9/5   & 32/2/16 & 29/8/13 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Web/Unsure/NoWeb Evaluations}
%     \label{tab:evaluations}
% \end{table}

\begin{table}[t]
    \centering

    \begin{tabular}{lcccc}
        \toprule
        && \multicolumn{3}{c}{Evaluation Model} \\
        \cmidrule(r){3-5}  
        & & GPT & Claude & Gemini \\
        \midrule
        \multirow{3}{*}{claim1}
        & GPT    & 78 (2)  & 78 (0) & 76 (0) \\
        &Claude & 68 (8) & 68 (4) & 70 (14)  \\
        &Gemini & 76 (6)  & 60 (4) & 64 (8)\\
        \midrule
        \multirow{3}{*}{claim2}
        &GPT   & 78 (10)  & 62 (6) & 64 (0) \\
        &Claude  & 58 (18)   & 56 (12)  & 64 (6)  \\
        &Gemini & 72 (18)   & 64 (4) & 54 (16) \\
        \bottomrule
    \end{tabular}
    \caption{Web/Unsure/NoWeb Evaluations}
    \label{tab:evaluations}
\end{table}


==> tables/performance_compare.tex <==

% \begin{table}[t]
% \ifdiff
% \begin{mdframed}[backgroundcolor=blue!20]
% \fi
% \centering
% \caption{Comparison of performance by model.}
% \label{tab:exp_summary}
% \footnotesize
% \begin{tabular}{ccccc}
% \toprule
% Task & GPT & Claude & Gemini \\
% \midrule
% \makecell{PII collection\\(Section~\ref{sec:pii_collection})}
% &  &  & N/A\\
% \midrule
% \makecell{Impersonation post\\generation\\(Section~\ref{sec:impersonation})} 
% & 93.9 & 85.7 & 74.0\\
% \midrule
% \makecell{Spear-phishing email\\generation\\(Section~\ref{sec:phishing})}  
% & 25.0 & 33.3 & N/A\\
% \bottomrule
% \end{tabular}
% \ifdiff
% \end{mdframed}
% \fi
% \end{table}




\begin{table}[h]
\ifdiff
\begin{mdframed}[backgroundcolor=blue!20]
\fi
\centering
\caption{Performance comparison of models across different tasks. Results for PII collection involving the professor group and impersonation post generation for claim 1 were obtained using WebNav agents. Results for spear-phishing email generation (login credential purpose) were from WebSearch agents.}
\label{tab:performance_compare}
\footnotesize
% \setlength{\tabcolsep}{4pt}
\begin{tabular}{cccc}
\toprule
Task & Metric & GPT & Claude \\
\midrule
\multirow{5}{*}{\makecell{PII collection\\(Section~\ref{sec:pii_collection})}}
& \# name & 570 & 612 \\
& \# phone & 407 & 382 \\
& \# office & 520 & 542\\
& \# email & 547 & 579\\
& \# page & 443 & 563\\
\midrule
\makecell{Impersonation post\\generation\\(Section~\ref{sec:impersonation})} 
& \makecell{\% Yes\\(Yes/No test)} & 93.9 & 85.7 \\
\midrule
\makecell{Spear-phishing email\\generation\\(Section~\ref{sec:phishing})}  
& click-rate & 25.0 & 33.3\\
\bottomrule
\end{tabular}
\ifdiff
\end{mdframed}
\fi
\end{table}

==> tables/phishing_auth.tex <==
\begin{table*}[t]

\centering
\footnotesize
\caption{Survey results about perceived authenticity of phishing emails. Percentages represent responses relative to the total number of participants. }
\label{tab:overall_auth}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
 & &&& \multicolumn{5}{c}{Genuine or Phishing}  \\
\cmidrule(r){5-9}
    Model & Web use & Purpose & Sender's institution &\makecell{Definitely\\genuine} 
     & \makecell{Probably\\genuine} 
     & Unsure
     & \makecell{Probably\\phishing} 
     & \makecell{Definitely\\phishing} \\
\midrule
\multirow{4}{*}{Claude}
& o & general & not designated & 5.00 & 13.33 & 13.33  & 43.33 & 25.00  \\
& x & general & not designated  &5.00&18.33&6.67  & 21.67 & 48.33  \\
& o & credential &  not designated  & 3.33&25.00&10.00  & 26.67 & 35.00\\
& o & general & different from target's   & 3.33 & 25.00 & 26.67 &  35.00 & 10.00    \\
\midrule
\multirow{3}{*}{GPT} 
& o & general & not designated  &3.33&10.00&13.33 & 28.33 & 45.00\\
& x & general & not designated  & 1.67&8.33&13.33  & 28.33 & 48.33\\
& o & credential &  not designated   & 1.67&20.00&10.00 & 18.33 & 50.00\\
\midrule
\multicolumn{4}{c}{Average} & 3.33 & 17.14 & 13.33 & 28.81 & 37.38 \\
\bottomrule
\end{tabular}
\end{table*}







% 34.29 & 5.71 & 26.19 \\











==> tables/phishing_email_type_outdate.tex <==
\begin{table*}[ht]
\centering
\footnotesize
\caption{Types of LLM-crafted phishing emails. Percentages are relative to the number of participants.}
\begin{tabular}{c c c c c |cc c}
\toprule
\textbf{Type} & \textbf{Model} & \textbf{Web search} & \textbf{Email purpose} & \textbf{Sender's institution } &
\textbf{Move to spam (\%)} &
\textbf{Reply to email (\%)} &
\textbf{Click link (\%)} \\ 
\midrule
M1 & Claude & o & General & different from target's &
8.33 & 3.33 & \underline{46.67} \\
M2 & Claude & o & General & - &
23.33 & 6.67 & 26.67\\
M3 & Claude& o &  Login credentials & - &
35.00 & 6.67 & 33.33 \\
M4 & Claude& x & General & - &
40.00 & \underline{10.00} & 21.67\\
M5 & GPT& o & General & - & 
43.33 & 6.67 & 20.00\\
M6 & GPT & o & Login credentials & - &
\underline{46.67} & 5.00 & 25.00 \\
M7 & GPT & x & General & - & 
\underline{46.67} & 1.67 & 10.00\\
\midrule
&&&&Total & 34.29 & 5.71 & 26.19 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/post_generation.tex <==

\begin{table}[t]

\caption{Response generation capabilities of LLMs across different configurations based on the purpose of the claim or the nature of the target. successfully generated a response (o) or refused to generate a response (x)}
\label{tab:email_generation}
\footnotesize
\setlength{\tabcolsep}{1.3pt}
\begin{tabular}{cccccccc}
\toprule
&& \multicolumn{3}{c}{LLM} 
& \multicolumn{3}{c}{Agent} \\
\cmidrule(r){3-8}  
&& GPT& Claude & Gemini & GPT & Claude& Gemini\\
\midrule
\multirow{3}{*}{Claim} & General& o& o& x& o& o& x\\
& Credential & x& x& x& o& o& x\\
& Money& x& x& x& o& x& x\\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Email\\address\\
\end{tabular}}
& Institutional & o& o& x& o& o& x\\
& Gmail & o& x& x& o& o& x\\
\bottomrule
\end{tabular}
\end{table}


==> tables/professor_PII_navigation.tex <==
% \begin{table}[t]
% \centering
% \caption{Quantities of successfully collected PII using LLM agents with and without the navigation function. GPT and Claude agents retrieve PII for 256 and 417 professors, respectively.}
% \label{tab:pii_navi}
% \footnotesize
% % \setlength{\tabcolsep}{2pt}
% \begin{tabular}{ccccc}
% \toprule
% & \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{Claude} \\
% \cmidrule(r){2-5}  
% navigation & x &o & x & o  \\
% \midrule
% phone & 96 & 144 & 122 & 219 \\
% office & 127 & 198 & 165 & 325 \\
% email & 217 & 211 & 342& 376 \\
% page & 166 & 145 & 302& 364\\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Quantities of successfully collected PII using LLM agents with and without the navigation function. GPT and Claude agents retrieve PII for 256 and 417 professors, respectively.}
% \label{tab:pii_navi}
% \footnotesize
% \setlength{\tabcolsep}{3.5pt}
% \begin{tabular}{ccccccc}
% \toprule
% &navigation&names&phone & office & email & page\\
% \midrule
% &x&\multirow{2}{*}{256}&96 & 127 & 217 & 166 \\
% GPT&o&&144 & 198& 211& 145 \\
% \cmidrule(r){3-7}
% && &48&71&-6&-21\\ 
% \midrule
% &x&\multirow{2}{*}{417}&122 & 165& 342& 302\\
% Claude
% &o&&219 & 325& 376 & 364\\
% \cmidrule(r){3-7}
% && &97&160&34&62\\ 
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[t]
\centering
\caption{Quantities of successfully collected PII using LLM agents with and without the navigation function. GPT and Claude agents retrieve PII for 256 and 417 professors, respectively.}
\label{tab:pii_navi}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{ccccccc}
\toprule
&navigation&target&phone & office & email & page\\
\midrule
\multirow{2}{*}{GPT}&x&\multirow{2}{*}{256}&96 & 127 & 217 & 166 \\
&o&&144 & 198& 211& 145 \\
\midrule
\multirow{2}{*}{Claude}&x&\multirow{2}{*}{417}&122 & 165& 342& 302\\
&o&&219 & 325& 376 & 364\\ 
\bottomrule
\end{tabular}
\end{table}


==> tables/professor_self_eval.tex <==
% \begin{table}[t]
% \centering
% \footnotesize
% \caption{Self-evaluation results regarding the professor \textit{name}. *Recall exceeds 1 due to the identification of professors specializing in CS-related fields but not listed on the official CS faculty pages.}
% \label{tab:professor_self_eval}
% \begin{tabular}{cccccc}
% \toprule
% && \multicolumn{2}{c}{GPT} & \multicolumn{2}{c}{Claude} \\
% \cmidrule(r){3-6} 
% & Self-eval & x& o  &x & o \\   
% \midrule
% \multirow{3}{*}{LLM} 
% & TP& 327& 265& 795& 663\\
% & Precision & 0.389& 0.765 & 0.574 & 0.719  \\
% & Recall & 0.477& 0.386 & 1.159* & 0.966  \\
% \midrule
 
% \multirow{3}{*}{WebSearch agent}
% & TP& 506& 431& 632 & 552 \\
% & Precision & 0.496& 0.872& 0.754 & 0.936 \\
% & Recall & 0.738 & 0.628 & 0.921 & 0.805  \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[t]
\centering
\footnotesize
\caption{Self-evaluation results regarding the professor \textit{name}.}
\label{tab:professor_self_eval}
\begin{tabular}{ccccc}
\toprule
& \multicolumn{2}{c}{LLM} & \multicolumn{2}{c}{WebSearch agent} \\
\cmidrule(r){2-5} 
Self-eval & x& o  &x & o \\   
\midrule
 TP& 327& 265& 506& 431 \\
 Precision & 0.389& 0.765 & 0.496& 0.872 \\
Recall & 0.477& 0.386 &  0.738 & 0.628 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/student_name_collection.tex <==
\begin{table}[t]
\centering
\caption{Precision and Recall of the collected names for CS students.}
\label{tab:student_prc_result}
\footnotesize
\begin{tabular}{cccccc}
\toprule
&&\multicolumn{3}{c}{Tools} \\
\cmidrule(r){3-5}
&& None & Search & Navigation \\
\midrule
\multirow{2}{*}{GPT} &Precision & 0.002 & 0.062 & 0.990\\
&Recall&  0.007 & 0.252 & 0.990\\
\midrule
\multirow{2}{*}{Claude} &Precision& 0.0117 & 0.054 & 0.901 \\
&Recall & 0.018 & 0.491 & 0.935\\
\bottomrule
\end{tabular}
\end{table}


